Carbon Regulation and Competition in the European Airline Industry

The European Union Emissions Trading System is set to substantially increase the effective carbon price faced by airlines. We estimate a two-stage model of airline competition with endogenous product entry, direct departure frequencies, and pricing. Impacts are highly asymmetric across carrier types and market segments. Consumer surplus declines by up to 34% overall and up to 95% in medium- and long-haul markets. Short-haul markets gain welfare as airlines reallocate capacity toward shorter routes. Airline profits decline by 1--42%, but carbon tax revenue of $1.9--2.9 billion and the social value of avoided emissions of $2.7--4.0 billion more than offset private-surplus losses.

==> tables/market_share.tex <==
\begin{table}[htbp]
\centering
\caption{Market Share Conditional on Travel}
\label{tab:market_share}
\begin{tabular}{lcccc}
\toprule
& \textbf{2016} & \textbf{2017} & \textbf{2018} & \textbf{2019} \\
\midrule
\textbf{Low-cost} & 56.49\% & 55.97\% & 55.53\% & 56.36\% \\
\textbf{Full-service} & 43.51\% & 44.03\% & 44.47\% & 43.64\% \\
\bottomrule
\end{tabular}
\end{table}

